An Approach to the Analysis of the South Slavic Medieval Labels Using Image Texture

The paper presents a new script classification method for the discrimination of the South Slavic medieval labels. It consists in the textural analysis of the script types. In the first step, each letter is coded by the equivalent script type, which is defined by its typographical features. Obtained coded text is subjected to the run-length statistical analysis and to the adjacent local binary pattern analysis in order to extract the features. The result shows a diversity between the extracted features of the scripts, which makes the feature classification more effective. It is the basis for the classification process of the script identification by using an extension of a state-of-the-art approach for document clustering. The proposed method is evaluated on an example of hand-engraved in stone and hand-printed in paper labels in old Cyrillic, angular and round Glagolitic. Experiments demonstrate very positive results, which prove the effectiveness of the proposed method.

==> refs.tex <==
\begin{thebibliography}{5}
%

\bibitem {Zhang2013}
Zhang, H., Zhao, K., Song, Yi-Zhe, Guo, J.:
Text extraction from natural scene image: A survey.
Neurocomputing 122(0), 310--323 (2013)

\bibitem {Fucic82}
Fu\v ci\'c, B.:
Glagoljski natpisi (in english "Glagolitic Labels"), Jugoslovenska akademija znanosti i umjetnosti.
Zagreb, (1982)

\bibitem {BrodicSC}
Brodi\'c, D., Milivojevi\'c, Z.N., Maluckov, \v C.A.:
An approach to the script discrimination in the Slavic documents.
Soft Computing, 1--11, In Press, DOI: 10.1007/s00500-014-1435-1

\bibitem {Brodic14}
Brodi\'c, D., Maluckov, \v C.A., Milivojevi\'c, Z.N., Draganov I.R.:
Differentiation of the script using adjacent local binary patterns.
AIMSA 2014. LNCS, vol. 8722, 162--169, Springer, Heidelberg (2014)

\bibitem {Preparata95}
Preparata, F. P., Shamos, M. I.:
Computational Geometry: An Introduction.
Springer, Berlin (1995).

\bibitem {Zram98}
Zramdini A.W., Ingold, R.:
Optical font recognition using typographical features.
IEEE Transaction on Pattern Analysis and Machine Intelligence 20(8), 877--882 (1998)

\bibitem {Tan98}
Tan, X.:
Texture information in run-length matrices.
IEEE Transaction on Image Processing 7(11), 1602--1609 (1998)

\bibitem{Galloway75}
Galloway, M.M.:
Texture analysis using gray level run lengths.
Computer, Graphics and Image Processing  4(2), 172--179 (1975)

\bibitem{Chu90}
Chu, A., Sehgal, C.M., Greenleaf, J.F.:
Use of gray value distribution of run lengths for texture analysis.
Pattern Recognition Letters 11(6), 415--419 (1990)

\bibitem{Dasar91}
Dasarathy, B.R., Holder, E.B.:
Image characterizations based on joint gray-level run-length distributions.
Pattern Recognition Letters, 12(8), 497--502 (1991)

\bibitem{Ojala96}
Ojala, T., PietikŠinen, M., Harwood, D.:
A comparative study of texture measures with classification based on feature distributions.
Pattern Recognition 29, 51--59 (1996)

\bibitem{Ojala2002}
Ojala, T., PietikŠinen, M., MŠenpŠŠ, T.:
Multi-resolution gray-scale and rotation invariant texture classification with local binary patterns.
IEEE Transaction on Pattern Analysis and Machine Intelligence 24, 971--987 (2002)

\bibitem{Amelio14}
Amelio, A., Pizzuti, C.:
A new evolutionary-based clustering framework for image databases.
ICISP 2014. LNCS, vol. 8509, 322--331, Springer International Publishing (2014)

\bibitem{Marti2001}
Marti, R., Laguna, M., Glover, F., Campos, V.:
Reducing the bandwidth of a sparse matrix with tabu search.
European Journal of Operational Research 135(2), 450--280 459 (2001)

\bibitem{Yuyu13}
Yuyu, Y., Xu, W., Yueming, L.:
A Hierarchical Method for Clustering Binary Text Image.
Trustworthy Computing and Services, CCIS 320, pp. 388--396, Springer (2013)

\bibitem{Aggar12}
Aggarwal, C. C., Zhai, C.:
A Survey of Text Clustering Algorithms.
In Aggarwal, C. C. et al (eds.), Mining Text Data, Springer US, pp. 77--128 (2012).

\bibitem{Zhu2006}
Zhu, Q., Li, J., Zhou, G., Li, P., Qian, P.:
A Novel Hierarchical Document Clustering Algorithm Based on a kNN Connection Graph.
ICCPOL 2006. LNAI, vol. 4285, 120--130, Springer, Heidelberg (2006)

\bibitem{Andrews2007}
Andrews, N.O., Fox, E.A.:
Recent Developments in Document Clustering.
Tech. rep., Computer Science, Virginia Tech (2007)

\bibitem{Vries12}
Vries, C.M.D., Geva, S., Trotman, A.:
Document clustering evaluation: Divergence from a random baseline.
CoRR abs/1208.5654 (2012)

\bibitem{Mann2009}
Manning, C.D., Raghavan, P., Schutze, H.:
Introduction to Information Retrieval.
Cam-bridge University Press, Online edition (2009)

\end{thebibliography}

